Timestep Rescheduling in Diffusion Inversion

Diffusion inversion, which maps images back to the Gaussian latent space of a diffusion model, is a critical task for image reconstruction and editing. While DDIM enables fast deterministic inversion, it inherently introduces deviations that accumulate into noticeable inversion errors. Existing methods often address this by solving a fixed-point problem but largely overlook how the selection of the diffusion timestep in the noise scheduler influences inversion fidelity. In this work, we reveal that the deviation scale in diffusion inversion is strongly dependent on the timestep size, and exhibits a parabolic trend, with larger errors concentrated at both small and large timesteps. Based on this finding, we propose a simple yet effective nonuniform timestep scheduler that integrates a global rescaling with a local dynamic programming based rescheduling, enabling a strategic allocation of computational effort that minimizes the overall inversion error and preserves higher inversion accuracy. Our method serves as an off-the-shelf enhancement for existing inversion techniques and requires no extra parameters or computational overhead. Through extensive experiments, we verify that integrating our scheduler consistently boosts the performance of existing inversion methods, achieving superior results in image reconstruction and editing.

==> fig_tex/editing/edit_1.tex <==
\begin{figure*}[t]
% \captionsetup{font={scriptsize}}
  \centering
  \rotatebox{90}{\scriptsize{~~~~~~~~~~~~~~~~~~~~Source}}
  \subfloat{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/input_000000000006.jpg}}
  \hfill
  \subfloat{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/input_000000000030.jpg}}
  \hfill
  \subfloat{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/input_000000000040.jpg}}
  \hfill
  \subfloat{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/input_000000000043.jpg}}
  \hfill
  \subfloat{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/input_000000000122.jpg}}

  \centering
  \rotatebox{90}{\scriptsize{~~~~~~~~~~~~~~~~~~ReNoise}}
  \subfloat{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/ReNoise_000000000006.jpg}}
  \hfill
  \subfloat{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/ReNoise_000000000030.jpg}}
  \hfill
  \subfloat{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/ReNoise_000000000040.jpg}}
  \hfill
  \subfloat{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/ReNoise_000000000043.jpg}}
  \hfill
  \subfloat{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/ReNoise_000000000122.jpg}}
  
  \centering
  \rotatebox{90}{\scriptsize{~~~~~~~~~~~~~~~~~~w/ Ours}}
  \subfloat[``...\sout{tulip} lion...'']{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/ReNoise_wOurs_000000000006.jpg}}
  \hfill
  \subfloat[``...\sout{stream} road...'']{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/ReNoise_wOurs_000000000030.jpg}}
  \hfill
  \subfloat[``...putting hands down...'']{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/ReNoise_wOurs_000000000040.jpg}}
  \hfill
  \subfloat[``\sout{large red} small blue boat'']{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/ReNoise_wOurs_000000000043.jpg}}
  \hfill
  \subfloat[``... in \sout{snow} leaves ...'']{\includegraphics[width=0.194\linewidth]{figs/editing/0_random/ReNoise_wOurs_000000000122.jpg}}
  % \centering
  % \subfloat[{\scriptsize SpacCNN\cite{Chen2018RobustCNN}}]{\label{fig:syn1-e}\includegraphics[width=0.194\linewidth]{figures/results/NTURain/syn1/5_SpacCNN.jpg}}
  % \hfill
  % \subfloat[{\scriptsize SLDNet\cite{Yang2020Self}}]{\label{fig:syn1-f}\includegraphics[width=0.194\linewidth]{figures/results/NTURain/syn1/6_SLDNet.jpg}}
  % \hfill
  % \subfloat[{\scriptsize S2VD\cite{Yue2021Semi}}]{\label{fig:syn1-g}\includegraphics[width=0.194\linewidth]{figures/results/NTURain/syn1/7_S2VD.jpg}}
  % \hfill
  % \subfloat[{\scriptsize Ours}]{\label{fig:syn1-h}\includegraphics[width=0.194\linewidth]{figures/results/NTURain/syn1/8_Ours.jpg}}

% \setlength{\abovecaptionskip}{1pt} 
% \setlength{\belowcaptionskip}{-17pt}
  \caption{Visualization results comparing our method with ReNoise~\cite{garibi2024renoise} for improving inversion and editing techniques on PIE-Bench~\cite{ju2023direct}. The first row shows the source images, the second row displays the results of ReNoise~\cite{garibi2024renoise}, and the third row presents our results.}
  \label{fig:renoise}
% \setlength{\abovecaptionskip}{-15pt} 
% \setlength{\belowcaptionskip}{-15pt}
% \vspace{-0.4cm}
\end{figure*}

